GPIRT: A Gaussian Process Model for Item Response Theory

The goal of item response theoretic (IRT) models is to provide estimates of latent traits from binary observed indicators and at the same time to learn the item response functions (IRFs) that map from latent trait to observed response. However, in many cases observed behavior can deviate significantly from the parametric assumptions of traditional IRT models. Nonparametric IRT models overcome these challenges by relaxing assumptions about the form of the IRFs, but standard tools are unable to simultaneously estimate flexible IRFs and recover ability estimates for respondents. We propose a Bayesian nonparametric model that solves this problem by placing Gaussian process priors on the latent functions defining the IRFs. This allows us to simultaneously relax assumptions about the shape of the IRFs while preserving the ability to estimate latent traits. This in turn allows us to easily extend the model to further tasks such as active learning. GPIRT therefore provides a simple and intuitive solution to several longstanding problems in the IRT literature.

==> tables/held-out.tex <==
\begin{table*}

\footnotesize
    \caption{Fit for GPIRT and the 2PL models with data held out. $\varepsilon \approx 2.2 \times 10^{-16}$ is machine epsilon.} 
    \label{tab:held-out}

\begin{center}
    \begin{tabular}{lp{1in}rrrr}
        \toprule
        & & \multicolumn{2}{c}{NPI} & \multicolumn{2}{c}{Congress} \\
        \cmidrule{3-4} \cmidrule(lr){5-6}
        \multicolumn{1}{c}{Hold out} &
        \multicolumn{1}{c}{Statistic} &
        \multicolumn{1}{c}{GPIRT} &
        \multicolumn{1}{c}{2PL} &
        \multicolumn{1}{c}{GPIRT} &
        \multicolumn{1}{c}{2PL} \\ 
        \midrule
            \multirow{6}{*}{10\%}   & Mean $\mathcal{L}$    & $-4169$   &  $-5797$              &  $-3208$ & $-3201$    \\
                                & Mean $\mathcal{L}$ / N    & $-0.5211$ & $-0.7246$             & $-0.123$ & $-0.122$ \\
                                & Diff.\ in means            & \multicolumn{2}{c}{$0.2035$}      & \multicolumn{2}{c}{$-0.0003$} \\
                                & (paired $t$-test)         & \multicolumn{2}{c}{($p < \varepsilon$)} & \multicolumn{2}{c}{($p = 0.53$)} \\
                                & Mean accuracy             & $0.738$   & $0.627$               & $0.957$   & $0.953$ \\
                                & Mean AUC                   & $0.816$   & $0.659$               & $0.991$   & $0.990$ \\[0.5em]
        \multirow{6}{*}{20\%}   & Mean $\mathcal{L}$        & $-8335$   & $-11605$              & $-6466$   & $-6443$              \\ 
                                & Mean $\mathcal{L}$ / N    & $-0.5210$ & $-0.7253$            , & $-0.124$  & $-0.123$             \\
                                & Diff.\ in means            & \multicolumn{2}{c}{$0.2043$}      & \multicolumn{2}{c}{$-0.0004$} \\
                                & (paired $t$-test)         & \multicolumn{2}{c}{($p < \varepsilon$)} & \multicolumn{2}{c}{($p = 0.09$)} \\
                                & Mean accuracy             & $0.739$   & $0.625$               & $0.957$   & $0.953$ \\
                                & Mean AUC                  & $0.817$   & $0.664$               & $0.991$   & $0.990$ \\
        \bottomrule
    \end{tabular}
\end{center}

Mean  $\mathcal{L}$ is the average log-likelihood across the 20 replications where the held out sample is 10\% or 20\%. Mean $\mathcal{L}$ / N is the mean  $\mathcal{L}$ divided by the number of responses held out.  Mean accuracy  is the proportion correctly classified of the held out responses.
\end{table*}

